The HST view of the innermost narrow line region

We analyze the properties of the innermost narrow line region in a sample of low-luminosity AGN. We select 33 LINERs (bona fide AGN) and Seyfert galaxies from the optical spectroscopic Palomar survey observed by HST/STIS. We find that in LINERs the [NII] and [OI] lines are broader than the [SII] line and that the [NII]/[SII] flux ratio increases when moving from ground-based to HST spectra. This effect is more pronounced considering the wings of the lines. Our interpretation is that, as a result of superior HST spatial resolution, we isolate a compact region of dense ionized gas in LINERs, located at a typical distance of about 3 pc and with a gas density of about 10$^4$-10$^5$ cm$^{-3}$, which we identify with the outer portion of the intermediate line region (ILR). Instead, we do not observe these kinds of effects in Seyferts; this may be the result of a stronger dilution from the NLR emission, since the HST slit maps a larger region in these sources. Alternatively, we argue that the innermost, higher density component of the ILR is only present in Seyferts, while it is truncated at larger radii because of the presence of the circumnuclear torus. The ILR is only visible in its entirety in LINERs because the obscuring torus is not present in these sources.

==> tab0.tex <==
\begin{table*}
\caption{The sample galaxies and log of the HST/STIS observations.}
\begin{tabular}{l|c|c|c|c|c|l|l|l}
\hline
Name &  D & $\sigma_{\star}$ & log L$_{\oiii}$ & Slit width
& Obs. Date& Obs. Id & Exp. Time & Scale \\
     &  [Mpc] & [km s$^{-1}$] & [erg s$^{-1}$] & [arcsec] & & & [s] & [\AA/pix]\\
\hline
\multicolumn{9}{l}{Liners Type 1}\\
\hline
NGC~3031  &  1.4  & 162 &  37.72  &0.1$\arcsec$ &1999-07-14 & O51301010        &1000 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~3998  & 21.6  & 305 &  39.62  &0.1$\arcsec$ &2002-04-07 & O6N902010 to 40  & 520 \,\,\,\,\,\,\,\,  & 1.11 \,\,\,\,\,\,\,\,\\
NGC~4203  &  9.7  & 167 &  38.53  &0.2$\arcsec$ &1999-04-18 & O4E010010 to 30  &2779 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~4450  & 16.8  & 135 &  38.78  &0.2$\arcsec$ &1999-01-31 & O4E016010 to 30  &2697 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~4579  & 16.8  & 165 &  39.42  &0.2$\arcsec$ &1999-04-21 & O57208040	       &2692 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\ 
\hline                              
\multicolumn{9}{l}{Liners Type 2}\\
\hline                              
NGC~0315  & 65.8  & 304 &  39.44  &0.1$\arcsec$ &2000-06-18 & O5EE02060 to 70 &  500 \,\,\,\,\,\,\,\,  & 1.11 \,\,\,\,\,\,\,\,\\
NGC~1052  & 17.8  & 215 &  40.10  &0.2$\arcsec$ &1999-01-02 & O57203050       & 1974 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~1961  & 53.1  & 165 &  39.11  &0.2$\arcsec$ &2001-12-27 & O6F450030 to 40 & 4963 \,\,\,\,\,\,\,\,  & 1.11 \,\,\,\,\,\,\,\,\\ 
NGC~2787  & 13.0  & 202 &  38.37  &0.2$\arcsec$ &1998-12-05 & O4E002010 to 30 & 2012 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~2911  & 42.2  & 243 &  39.34  &0.1$\arcsec$ &1998-12-03 & O4D311020       &  486 \,\,\,\,\,\,\,\,  & 1.11 \,\,\,\,\,\,\,\,\\ 
%NGC~3368  &  8.1  & 128 &  37.64  &0.2$\arcsec$ &1998-10-31 & O4E004010 to 30 & 2703 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\ 
NGC~3642  & 27.5  &  85 &  38.96  &0.2$\arcsec$ &2000-10-13 & O5H720030 to 40 &  864 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~4036  & 24.6  & 215 &  39.16  &0.2$\arcsec$ &1999-03-25 & O57206030       & 2896 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~4143  & 17.0  & 205 &  38.81  &0.2$\arcsec$ &1999-03-20 & O4E009010 to 30 & 2856 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~4258  &  6.8  & 148 &  38.76  &0.2$\arcsec$ &2001-03-16 & O67104030	      & 1440 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\ 
NGC~4278  &  9.7  & 261 &  38.88  &0.1$\arcsec$ &2000-05-11 & O57207030       & 3128 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~4477  & 16.8  & 177 &  38.82  &0.2$\arcsec$ &1999-04-23 & O4E018010 to 30 & 2613 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~4486  & 16.8  & 332 &  39.07  &0.1$\arcsec$ &2011-06-07 & OBIm01030 to 50 & 1717 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\ 
NGC~4548  & 16.8  & 113 &  38.11  &0.2$\arcsec$ &1999-04-26 & O4E020010 to 30 & 2673 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\ 
%NGC~4636  & 17.0  & 203 &  38.09  &0.2$\arcsec$ &2001-04-02 & O5L204020 to 30 & 3590 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
%NGC~4736  &  4.3  & 112 &  37.42  &0.1$\arcsec$ &2002-07-15 & O67110030 to 40 & 3922 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\ 
NGC~5005  & 21.3  & 172 &  39.41  &0.2$\arcsec$ &2000-12-24 & O5H741030       &  734 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~5077  & 40.6  & 255 &  39.52  &0.1$\arcsec$ &1998-03-12 & O4D305020       &  418 \,\,\,\,\,\,\,\,  & 1.11 \,\,\,\,\,\,\,\,\\ 
NGC~5377  & 31.0  & 170 &  38.81  &0.1$\arcsec$ &2011-03-04 & OBIB05010 to 60 & 4510 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\ 
NGC~6500  & 39.7  & 214 &  39.90  &0.1$\arcsec$ &1998-11-03 & O4D307030       &  236 \,\,\,\,\,\,\,\,  & 1.11 \,\,\,\,\,\,\,\,\\ 
\hline                              
\multicolumn{9}{l}{Seyferts Type 1}\\
\hline                              
NGC~3227  & 20.6  & 136   & 40.68 &0.2$\arcsec$ &1999-01-31 &O57204040	       &1890 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\ 
NGC~3516  & 38.9  & 181   & 40.80 &0.2$\arcsec$ &2000-06-18 &O56C01020 to 40   &2116 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\
NGC~4051  & 17.0  &  89   & 40.18 &0.2$\arcsec$ &2000-03-12 &O5H730030 to 40   & 864 \,\,\,\,\,\,\,\,  & 1.11 \,\,\,\,\,\,\,\,\\ 
\hline                              
\multicolumn{9}{l}{Seyferts Type 2}\\
\hline                              
NGC~1358  & 53.6  & 222   & 40.84 &0.2$\arcsec$ &2002-01-25 &O6BU03010 to 30   &3000 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\, \\ 
NGC~1667  & 61.2  & 169   & 40.79 &0.2$\arcsec$ &2001-10-14 &O6BU04010 to 30   &3000 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\, \\
NGC~2273  & 28.4  & 149   & 40.43 &0.2$\arcsec$ &2001-11-04 &O6BU05010 to 30   &3266 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\, \\ 
NGC~3982  & 17.0  &  73   & 39.83 &0.2$\arcsec$ &1998-04-11 &O4E006010 to 30   &2997 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\,\\  
NGC~4501  & 16.8  & 167   & 39.10 &0.2$\arcsec$ &1999-04-26 &O4E019010 to 30   &2673 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\, \\  
NGC~4698  & 16.8  & 149   & 38.81 &0.2$\arcsec$ &1999-04-26 &O4E022010 to 30   &2673 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\, \\  
NGC~5194  &  7.7  &  96   & 38.91 &0.2$\arcsec$ &2002-04-03 &O6FM01010 to 50   &10467 \,\,\,\,\,\,\,\,  & 1.11 \,\,\,\,\,\,\,\,\\
NGC~6951  & 24.1  & 128   & 38.69 &0.2$\arcsec$ &2000-06-17 &O5H752030 to 40   &864 \,\,\,\,\,\,\,\,  & 0.55 \,\,\,\,\,\,\,\, \\ 
\hline
\end{tabular}
\label{table0}
\medskip

\small{(1) Object name;
  (2) distance of the source from \citet{ho95};  (3) stellar
  velocity dispersion from \citet{ho09a};  
  (4) Logarithm of the nuclear [OIII] emission line luminosity from  \citet{ho97}; from (5) to (9) HST data description.}
\end{table*}
\medskip
  


==> tab1.tex <==
\begin{table}
\caption{Line widths comparisons}
\begin{tabular}{l|c|c|c|c|}
\hline
     & \multicolumn{2}{|c|}{LINERs} & \multicolumn{2}{|c|}{Seyferts}\\ 
\hline
     & Median & Average & Median & average \\
\hline
\sii\ Palomar                    &    386 &    412  &    236 &    273 \\ 
\sii\ HST                          &    463 &    518  &    226 &    236 \\ 
\sii\ HST{\tiny(10-90)\%} &    738 &    794  &    358 &    345 \\ 
\nii\ Palomar                    &    389 &    440  &    243 &    270 \\ 
\nii\ HST                          &    564 &    583  &    252 &    252 \\ 
\nii\ HST{\tiny(10-90)\%} &    944  &   1041&    400 &    404 \\ 
\oi\  HST                          &    636 &    739  &    232 &    238 \\ 
\hline
\end{tabular}
\label{tab1}

\medskip
\small{All widhts are in \kms.} 
\end{table}
\medskip











  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
 




 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 



 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 

 
 
 
 
 


==> tab3.tex <==
\landscape
\begin{table}
\caption{Forbidden line measurements}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline\hline
Name & \multicolumn{7}{|c|}{[SII]}  
     & \multicolumn{7}{|c|}{[NII]} 
     & \multicolumn{2}{|c|}{[OI]}  \\
\hline
     & \multicolumn{4}{|c|}{HST} & \multicolumn{3}{|c|}{Palomar} 
     & \multicolumn{4}{|c|}{HST} & \multicolumn{3}{|c|}{Palomar} 
     & \multicolumn{2}{|c|}{HST} \\
\hline
     & Flux & FWHM & v90-v10 & r
     & Flux & FWHM & r
     & Flux & FWHM & v90-v10 & r
     & Flux & FWHM & r
     & Flux & FWHM \\
\hline
\multicolumn{17}{l}{Liners Type 1}\\
\hline
3031 & -13.42 &    436  &    443  & 0.59 & -12.75 &    230 & 0.92  & -12.82 &    539  &    875  & 0.40 & -12.55 &    273  & 0.43 & -13.04 &    461  \\
3998 & -13.05 &    707  &   1626  & 0.79 & -12.75 &    439 & 1.14  & -12.75 &    968  &   1304  & 0.91 & -12.63 &    460  & 0.82 & -12.62 &   1326  \\
4203 & -13.83 &    256  &    434  & 0.75 & -13.58 &    371 & 1.01  & -13.29 &    441  &    768  & 0.90 & -13.36 &    372  & 0.75 & -13.28 &    592  \\
4450 & -13.69 &    368  &    491  & 0.84 & -13.38 &    311 & 1.01  & -13.61 &    416  &    630  & 0.73 & -13.51 &    312  & 0.47 & -13.49 &    653  \\
4579 & -13.80 &    536  &    848  & 0.74 & -12.92 &    388 & 1.10  & -13.61 &    565  &    701  & 0.30 & -12.84 &    390  & 0.51 & -13.54 &    980  \\
\hline
\multicolumn{17}{l}{Liners Type 2}\\
\hline 
 315 & -14.46 &    611  &    805  & 0.73 & -13.96 &    386 & 1.22  & -13.90 &    858  &   1377  & 0.31 & -13.56 &    436  & 0.43 &     -- &      -- \\
1052 & -13.44 &    572  &    739  & 0.74 & -12.18 &    509 & 1.13  & -13.31 &    646  &   1579  & 1.29 & -12.20 &    618  & 0.93 & -13.31 &    637  \\
1961 & -14.65 &    418  &    752  & 0.88 & -13.69 &    386 & 1.22  & -14.45 &    493  &    766  & 0.40 & -13.45 &    384  & 0.59 & -14.97 &    514  \\
2787 & -14.08 &    508  &    538  & 0.79 & -13.58 &    376 & 1.09  & -13.68 &    583  &   1255  & 0.44 & -13.35 &    403  & 0.68 &     -- &      -- \\
2911 & -15.49 &    371  &    417  & 1.23 & -13.33 &    485 & 1.28  & -15.05 &    704  &    999  & 0.34 & -13.26 &    499  & 0.59 &     -- &      -- \\
%3368 & -15.71 &    196  &    225  & 0.97 & -15.60 &    210 & 1.24  & -15.54 &    267  &    273  & 0.47 & -15.63 &    216  & 0.86 &     -- &      -- \\
3642 & -14.62 &    182  &    470  & 0.89 & -13.61 &    189 & 1.29  & -14.37 &    323  &    800  & 0.99 & -13.67 &    178  & 1.98 &     -- &      -- \\
4036 & -14.64 &    494  &    538  & 0.89 & -13.24 &    381 & 1.22  & -14.34 &    557  &    718  & 0.32 & -13.12 &    386  & 0.52 & -14.99 &    471  \\
4143 & -13.84 &    463  &    794  & 0.78 & -13.77 &    260 & 1.10  & -13.31 &    614  &   1366  & 0.42 & -13.32 &    360  & 0.86 & -13.84 &    669  \\
4258 & -13.92 &    401  &    500  & 0.78 & -13.39 &    324 & 1.05  & -13.52 &    708  &    912  & 1.63 & -13.21 &    348  & 1.39 & -13.78 &    459  \\
4278 & -14.62 &    780  &   1366  & 0.71 & -12.72 &    484 & 1.14  & -14.35 &    960  &   1824  & 0.62 & -12.70 &    506  & 0.88 & -14.69 &   1379  \\
4477 & -14.59 &    223  &    422  & 0.89 & -13.65 &    296 & 1.18  & -14.17 &    302  &    944  & 0.37 & -13.41 &    277  & 0.63 &     -- &      -- \\
4486 & -13.94 &   1547  &   1887  & 1.50 & -12.98 &   1139 & 1.50  & -13.47 &      -- &      -- & 0.28 & -12.74 &   1139  & 0.39 &     -- &      -- \\
4548 & -15.72 &    165  &    217  & 1.11 & -15.31 &     71 & 1.18  & -15.53 &    190  &    285  & 0.31 & -15.92 &    218  & 0.49 &     -- &      -- \\
%4636 & -15.99 &    537  &    536  & 0.85 & -14.08 &    330 & 1.37  & -15.72 &    603  &    962  & 0.31 & -14.01 &    357  & 0.78 &     -- &      -- \\
%4736 & -15.89 &    217  &    262  & 0.69 & -15.64 &    155 & 1.14  & -15.69 &    137  &    244  & 0.10 & -15.09 &    223  & 0.67 & -16.06 &    256  \\
5005 & -14.03 &    399  &    745  & 1.00 & -12.74 &    683 & 1.14  & -13.75 &    494  &    893  & 0.22 & -12.45 &    747  & 0.35 &     -- &      -- \\
5077 & -14.33 &    898  &   1279  & 0.69 & -13.54 &    492 & 1.29  & -14.18 &    871  &   1252  & 0.78 & -13.49 &    522  & 0.92 &     -- &      -- \\
5377 & -14.58 &    130  &    498  & 0.90 & -13.66 &    296 & 1.19  & -14.27 &    261  &   1397  & 0.23 & -13.51 &    313  & 0.38 &     -- &      -- \\
6500 & -14.49 &    933  &   1666  & 0.93 & -13.01 &    560 & 1.14  & -14.50 &    763  &   1220  & 1.22 & -13.12 &    548  & 1.37 &     -- &      -- \\
\hline
\multicolumn{17}{l}{Seyferts Type 1}\\
\hline
3227 & -13.69 &    272  &    464  & 0.70 & -12.49 &    499 & 0.94  & -13.37 &    257  &    336  & 1.24 & -12.24 &    446  & 0.58 & -13.84 &    233  \\
3516 & -15.09 &    246  &    238  & 0.62 & -13.20 &    311 & 0.93  & -14.17 &      -- &      -- & 4.21 & -12.76 &    312  & 1.05 & -15.59 &    188  \\
4051 & -14.82 &    187  &    304  & 0.71 & -12.96 &    235 & 0.98  & -14.14 &      -- &      -- & 6.63 & -12.59 &    235  & 2.04 &     -- &      -- \\
\hline
\multicolumn{17}{l}{Seyferts Type 2}\\
\hline
1358 & -14.08 &    395  &    373  & 0.93 & -13.17 &    256 & 1.15  & -13.74 &    441  &    463  & 0.43 & -12.87 &    271  & 0.55 & -14.46 &    417  \\
1667 & -14.33 &    330  &    479  & 0.80 & -13.12 &    367 & 1.03  & -13.87 &    332  &    595  & 0.44 & -12.74 &    377  & 0.44 &     -- &      -- \\
2273 & -13.71 &    148  &    306  & 0.70 & -12.92 &    206 & 0.99  & -13.41 &    120  &    345  & 0.74 & -12.68 &    205  & 1.26 & -13.98 &    156  \\
3982 & -15.25 &    267  &    438  & 0.83 & -13.58 &    236 & 0.83  & -15.03 &    322  &    523  & 0.91 & -13.38 &    236  & 1.26 & -15.21 &    280  \\
4501 & -14.42 &    196  &    359  & 1.06 & -13.64 &    205 & 1.04  & -14.00 &    230  &    400  & 0.38 & -13.26 &    192  & 0.50 &     -- &      -- \\
4698 & -14.64 &    227  &    467  & 1.01 & -13.85 &    208 & 1.12  & -14.39 &    252  &    486  & 0.72 & -13.73 &    213  & 0.84 &     -- &      -- \\
5194 & -14.69 &    146  &    162  & 0.86 & -13.07 &    227 & 0.96  & -14.12 &    157  &    271  & 0.38 & -12.51 &    243  & 0.36 & -15.22 &    154  \\
6951 & -14.57 &    190  &    206  & 0.82 & -13.57 &    248 & 0.98  & -14.10 &    159  &    215  & 0.22 & -13.16 &    243  & 0.40 &     -- &      -- \\
\hline
\hline
\end{tabular}
\label{bigtable}
\medskip
\small{ 
\caption{(1) Object name  
From HST spectra:  (2) \sii flux (3) FWHM(\sii) (4) ratio of the \sii doublet.
From Palomar spectra: (5) \sii flux (6) FWHM(\sii) (7) ratio of the \sii doublet.
From HST spectra:  (8) \nii flux (9) FWHM(\nii) (10) ratio of the \nii doublet  
From Palomar spectra: (11) \nii flux (12) FWHM(\nii) (13) ratio of the \nii doublet.
From HST spectra:  (14) \oi flux (15) FWHM(\oi)  
From Palomar spectra: (16) \oi flux (17) FWHM(\oi). Fluxes are in logarithmic units of erg cm$^{-2}$ s$^{-1}$ and the FWHM in units of km s$^{-1}$.}
 }
\end{table}
\medskip
\endlandscape 

 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 

































  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  































 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 


































  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
 




 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 



 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 

 
 
 
 
 

